Convergence of the Critical Planar Ising Interfaces to Hypergeometric SLE

We consider the planar Ising model in rectangle $(\Omega; x^L, x^R, y^R, y^L)$ with alternating boundary condition: $\ominus$ along $(x^Lx^R)$ and $(y^Ry^L)$, $\xi^R\in\{\oplus, \text{free}\}$ along $(x^Ry^R)$, and $\xi^L\in\{\oplus, \text{free}\}$ along $(y^Lx^L)$. We prove that the interface of critical Ising model with these boundary conditions converges to the so-called hypergeometric SLE$_3$. The method developed in this paper does not require constructing new holomorphic observable and the input is the convergence of the interface with Dobrushin boundary condition. This method could be applied to other lattice models, for instance Loop-Erased Random Walk and level lines of discrete Gaussian Free Field.

==> tex/open.tex <==
\subsection*{Question 1---Theorem \ref{thm::slepair_lessthan4} for $\kappa\in (4,8)$}
We believe the conclusion in Theorem \ref{thm::slepair_lessthan4} also holds for $\kappa\in (4,8)$, but the prove is unknown to our knowledge. Assume it holds for $\kappa\in (4,8)$, then by a similar proof of Theorem \ref{thm::ising_cvg_pair}, we can argue that the interface in critical FK-Ising model with alternating boundary condition (as in Proposition \ref{prop::fkising_cvg_pair}) converges to $\hSLE_{\kappa}$ with $\kappa=16/3$. 
\subsection*{Question 2---Theorem \ref{thm::slepair_lessthan4} Identification}
In Theorem \ref{thm::slepair_lessthan4} Identification part, we need to assume $\rho^L=0$, and we do not have an explicit driving function of the marginal law of $\eta^L$ when $\rho^L\neq 0$. In fact, to identify the marginal law of $\eta^L$ for $\rho^L\neq 0$ is related to the question on triple SLEs. 

Suppose $\Omega$ is a non-empty simply connected proper subset of $\C$ and $x^L, x^M, x^R, y^R, y^M, y^L$ are six boundary points in counterclockwise order. 
Fix $\kappa\in (0,4)$ and $\rho^L>-2, \rho^R>-2$. 
We can show that there exists a unique probability measure on the collection of disjoint triple curves $(\eta^L; \eta^M; \eta^R)$ where $\eta^L\in X_0(\Omega; x^L, y^L), \eta^M\in X_0(\Omega; x^M, y^M)$, and $\eta^R\in X_0(\Omega; x^R, y^R)$ such that  
\begin{itemize}
\item given $\eta^M$ and $\eta^R$, the conditional law of $\eta^L$ is $\SLE_{\kappa}(\rho^L)$;
\item given $\eta^L$ and $\eta^R$, the conditional law of $\eta^M$ is $\SLE_{\kappa}$;
\item given $\eta^L$ and $\eta^M$, the conditional law of $\eta^R$ is $\SLE_{\kappa}(\rho^R)$. 
\end{itemize}
However, we do not have an explicit driving function for the process $\eta^M$ under this unique measure. Denote by $\mu(\Omega; x^L, x^M, x^R, y^R, y^M, y^L; \kappa, \rho^L, \rho^R)$ the law of $\eta^M$ under this unique measure. 
Although we do not have an explicit expression for the law of $\eta^M$, we could still prove some nice consequences:
\begin{itemize}
\item The time reversal of $\eta^M$ is the same as $\mu(\Omega; y^R, y^M, y^L, x^L, x^M, x^R; \kappa, \rho^R, \rho^L)$.
\item Set $y^L=y^M=y^R$, then the law of $\eta^M$ degenerates to $\SLE_{\kappa}(\rho^L+2; \rho^R+2)$ with force points $(x^L; x^R)$. Hence 
the reversibility of the law of $\eta^M$ implies the reversibility of $\SLE_{\kappa}(\rho^L+2; \rho^R+2)$ when $x^L=x^M=x^R$.
\end{itemize}
\begin{comment}
\subsection*{Question 3---Hypergeometric SLE for $\rho\in (-4,\kappa/2-4)$}
In Section \ref{sec::hyperSLE}, we define and study $\hSLE_{\kappa}(\rho)$ for $\rho>-4$. We believe it is reversible for all $\rho>-4$, but we only prove it for $\rho\ge\kappa/2-4$ which is the range of $\rho$ such that the curve does hit the interval $[x,y]$. The reversibility would be more difficult to derive for the case when the curve may hit the interval $[x,y]$.  

Consider the critical Ising model in quad $(\Omega; x^L, x^R, y^R, y^L)$ with the boundary condition: $\oplus$ along $(y^Lx^L)$, $\ominus$ along $(x^Lx^R)$ and $(y^Ry^L)$, and $\free$ along $(x^Ry^R)$. Let $\eta$ be the interface starting from $x^L$ and ending at $y^L$. We have proved in Theorem \ref{thm::ising_cvg_pair} that, if we condition on the existence of a vertical crossing of $\ominus$, then the scaling limit of $\eta^L$ will converges to $\hSLE_3(-3/2)$. We believe that the scaling limit of $\eta^L$ (without conditioning on the vertical crossing) would be $\hSLE_3(-7/2)$. 
\end{comment}

==> tex/pre_probameasures.tex <==
Suppose $X$ is a metric space and $\LB_X$ is the Borel $\sigma$-field. Let $\LP$ be the space of probability measures on $(X, \LB_X)$. The Prohorov metric $d_{\LP}$ on $\LP$ is defined by  
\[d_{\LP}(\PP_1, \PP_2)=\inf\left\{\eps>0: \PP_1[A]\le \PP_2[A^{\eps}]+\eps, \PP_2[A]\le \PP_1[A^{\eps}]+\eps, \forall A\in\LB_X\right\}.\]
When $X$ is complete and separable, the space $\LP$ is complete and separable (\cite[Theorem 6.8]{BillingsleyConvergenceProbabilityMeasures}); moreover, a sequence $\PP_n$ in $\LP$ converges weakly to $\PP$ if and only if $d_{\LP}(\PP_n, \PP)\to 0$. 

Let $\Sigma$ be a family of probability measures on $(X,\LB_X)$. We call $\Sigma$ \textit{relatively compact} if every sequence of elements in $\Sigma$ contains a weakly convergent subsequence. We call $\Sigma$ \textit{tight} if, for every $\eps>0$, there exists a compact set $K_{\eps}$ such that $\PP[K_{\eps}]\ge 1-\eps$ for all $\PP\in\Sigma$. By Prohorov's Theorem (\cite[Theorem 5.2]{BillingsleyConvergenceProbabilityMeasures}), when $X$ is complete and separable, relative compactness is equivalent to tightness. 

==> tex/pre_sle.tex <==
We call a compact subset $K$ of $\overline{\HH}$ an \textit{$\HH$-hull} if $\HH\setminus K$ is simply connected. Riemann's Mapping Theorem asserts that there exists a unique conformal map $g_K$ from $\HH\setminus K$ onto $\HH$ such that
\[\lim_{|z|\to\infty}|g_K(z)-z|=0.\]
We call such $g_K$ the conformal map from $\HH\setminus K$ onto $\HH$ normalized at $\infty$.

\textit{Loewner chain} is a collection of $\HH$-hulls $(K_{t}, t\ge 0)$ associated with the family of conformal maps $(g_{t}, t\ge 0)$ obtained by solving the Loewner equation: for each $z\in\mathbb{H}$,
\[\partial_{t}{g}_{t}(z)=\frac{2}{g_{t}(z)-W_{t}}, \quad g_{0}(z)=z,\]
where $(W_t, t\ge 0)$ is a one-dimensional continuous function which we call the driving function. Let $T_z$ be the \textit{swallowing time} of $z$ defined as $\sup\{t\ge 0: \min_{s\in[0,t]}|g_{s}(z)-W_{s}|>0\}$.
Let $K_{t}:=\overline{\{z\in\mathbb{H}: T_{z}\le t\}}$. Then $g_{t}$ is the unique conformal map from $H_{t}:=\mathbb{H}\backslash K_{t}$ onto $\mathbb{H}$ normalized at $\infty$.

Here we discuss about the evolution of a point $y\in\R$ under $g_t$. We assume $y\ge 0$. There are two possibilities: if $y$ is not swallowed by $K_t$, then we define $Y_t=g_t(y)$; if $y$ is swallowed by $K_t$, then we define $Y_t$ to be the image of the rightmost of point of $K_t\cap\R$ under $g_t$. Suppose that $(K_t, t\ge 0)$ is generated by a continuous path $(\eta(t), t\ge 0)$ and that the Lebesgue measure of $\eta[0,\infty]\cap\R$ is zero. Then the process $Y_t$ is uniquely characterized by the following equation: 
\[Y_t=y+\int_0^t \frac{2ds}{Y_s-W_s},\quad Y_t\ge W_t,\quad \forall t\ge 0.\] 
In this paper, we may write $g_t(y)$ for the process $Y_t$. 

\textit{Schramm Loewner Evolution} $\SLE_{\kappa}$ is the random Loewner chain $(K_{t}, t\ge 0)$ driven by $W_t=\sqrt{\kappa}B_t$ where $(B_t, t\ge 0)$ is a standard one-dimensional Brownian motion.
In \cite{RohdeSchrammSLEBasicProperty}, the authors prove that $(K_{t}, t\ge 0)$ is almost surely generated by a continuous transient curve, i.e. there almost surely exists a continuous curve $\eta$ such that for each $t\ge 0$, $H_{t}$ is the unbounded connected component of $\mathbb{H}\backslash\eta[0,t]$ and that $\lim_{t\to\infty}|\eta(t)|=\infty$. There are phase transitions at $\kappa=4$ and $\kappa=8$: $\SLE_{\kappa}$ are simple curves when $\kappa\in [0,4]$; they have self-touching when $\kappa\in (4,8)$; and they are space-filling when $\kappa\ge 8$. 

It is clear that $\SLE_{\kappa}$ is scaling invariant, thus we can define $\SLE_{\kappa}$ in any simply connected domain $D$ from one boundary point $x$ to another boundary point $y$ by the conformal image: let $\phi$ be a conformal map from $\HH$ onto $D$ that sends $0$ to $x$ and $\infty$ to $y$, then define $\phi(\eta)$ to be $\SLE_{\kappa}$ in $D$ from $x$ to $y$. 
For $\kappa\in (0,8)$, the curves $\SLE_{\kappa}$ enjoys \textit{reversibility}: let $\eta$ be an $
 \SLE_{\kappa}$ in $D$ from $x$ to $y$, then the time-reversal of $\eta$ has the same law as $\SLE_{\kappa}$ in $D$ from $y$ to $x$. The reversibility for $\kappa\in (0,4]$ was proved in \cite{ZhanReversibility}, and it was proved for $\kappa\in (4,8)$ in \cite{MillerSheffieldIG3}. 
 
 \textit{Hypergeometric functions} are defined for $a,b\in\R$, $c\in\R\setminus\{0,-1,-2,-3,...\}$ and for $|z|<1$ by 
 \[\hF(a,b,c;z)=\sum_{n=0}^{\infty}\frac{(a)_n(b)_n}{n!(c)_n}z^n,\]
where $(q)_n$ is the Pochhammer symbol defined by $(q)_n=1$ for $n=0$ and $(q)_n=q(q+1)\cdots(q+n-1)$ for $n\ge 1$. 
When $c>a+b$, denote by $\Gamma$ the Gamma function, we have (see \cite[Equation (15.1.20)]{AbramowitzHandbook}),
\[\hF(a,b,c;1)=\frac{\Gamma(c)\Gamma(c-a-b)}{\Gamma(c-a)\Gamma(c-b)}.\]
The hypergeometric function is a solution of Euler's hypergeometric differential equation:
\[z(1-z)F''(z)+(c-(a+b+1)z)F'(z)-abF(z)=0.\]
In this section, we focus on 
\begin{equation}\label{eqn::hSLE_hyperF}
F(z):=\hF\left(\frac{4}{\kappa}, 1-\frac{4}{\kappa}, \frac{8}{\kappa};z\right).
\end{equation}
When $\kappa\in (0,8)$, we have $F(1)\in (0,\infty)$. In particular, $F$ is smooth for $z\in (-1,1)$ and is continuous for $z\in (-1,1]$. 

\begin{lemma}\label{lem::hypersle_mart}
Fix $\kappa\in (0,8)$, suppose $\eta$ is an $\SLE_{\kappa}$ in $\HH$ from 0 to $\infty$ and $(g_t,t\ge 0)$ is the corresponding family of conformal maps. Fix $0<x<y$ and let $T_x$ be the swallowing time of $x$. 
Define, for $t<T_x$,  
\[J_t=\frac{g_t'(x)g_t'(y)}{(g_t(y)-g_t(x))^{2}},\quad Z_t=\frac{g_t(x)-W_t}{g_t(y)-W_t}.\]
Let $F$ be defined through (\ref{eqn::hSLE_hyperF}). Then the following process is a local martingale:
\[M_t:=J_t^bZ_t^{2/\kappa}F(Z_t)\one_{\{t<T_x\}},\quad\text{where }b=\frac{6-\kappa}{2\kappa}.\]
\end{lemma}
\begin{proof}
By It\^{o}'s formula, one can check
\[dJ_t=\frac{-2J_t}{(g_t(y)-W_t)^2}\left(\frac{1}{Z_t}-1\right)^2dt,\quad dZ_t=\frac{(Z_t-1)dW_t}{g_t(y)-W_t}+\frac{(1-Z_t)(2+(2-\kappa)Z_t)dt}{Z_t(g_t(y)-W_t)^2}.\]
Therefore, the process $J_t^b\psi(Z_t)\one_{\{t<T_x\}}$ is a local martingale if $\psi$ is twice-differentiable and satisfies
\[\kappa z^2(1-z)\psi''(z)+2z(2+(2-\kappa)z)\psi'(z)-4b(1-z)\psi=0.\]
One can check that $\psi(z):=z^{2/\kappa}F(z)$ satisfies this ODE and hence $M_t$ is a local martingale. Moreover, we have
\[dM_t=M_t\left(\frac{2/\kappa}{W_t-g_t(x)}+\frac{-2/\kappa}{W_t-g_t(y)}-\frac{F'(Z_t)}{F(Z_t)}\left(\frac{1-Z_t}{g_t(y)-W_t}\right)\right)dW_t.\]
We will show that $M_t$ is actually a uniform integrable martingale in Proposition \ref{prop::hypersle_mart}. 
\end{proof}

\textit{$\SLE_{\kappa}(\underline{\rho})$ processes} are variants of $\SLE_{\kappa}$ where one keeps track of multiple points on the boundary. In this paper, we only need $\SLE_{\kappa}(\underline{\rho})$ processes with two force points on the boundary, to simplify the notations, we only introduce such processes. Fix two boundary points $0<x<y$ and two parameters $\rho,\nu\in\R$. $\SLE_{\kappa}(\rho,\nu)$ process with force points $(x,y)$ is the Loewner chain driven by $W$ which is the solution to the following system of integrated SDEs:
\begin{align}\label{eqn::sle_rho_sde}
W_t&=\sqrt{\kappa}B_t+\int_0^t\frac{\rho ds}{W_s-V_s^x}+\int_0^t\frac{\nu ds}{W_s-V_s^y},\\
V^x_t&=x+\int_0^t\frac{2ds}{V^x_s-W_s},\quad V^y_t=y+\int_0^t\frac{2ds}{V^y_s-W_s},\notag
\end{align}
where $B_t$ is one-dimensional Brownian motion. The process is well-defined up to the first time that $x$ is swallowed. 
The behavior of $\SLE_{\kappa}(\rho,\nu)$ varies according to different $\rho,\nu$, see \cite{MillerSheffieldIG1} and \cite[Lemma 15]{DubedatSLEDuality}. We list some of them that will be helpful later. 
\begin{itemize}
\item If $\rho>-2$ and $\rho+\nu>-2$, the process is well-defined for all time. If $\rho>-2$ and $\rho+\nu\le -2$, the process is well-defined up to the continuation threshold---the swallowing time of $y$ in this case. Moreover, the process is almost surely generated by a continuous curve up to and including the continuation threshold.
\item If $\rho\ge\kappa/2-2$, the curve never hits the interval $[x,y)$. If $\rho+\nu\ge \kappa/2-2$, the curve never hits the interval $[y,\infty)$. 
\item If $\rho>-2$ and $\rho+\nu\in (\kappa/2-4, \kappa/2-2)$, the curve hits the interval $(y,\infty)$ at finite time. 
\item If $\rho>-2$ and $\rho+\nu\le \kappa/2-4$, the curve accumulates at the point $y$ at finite time.
\end{itemize}
 
By Girsanov's Theorem, the law of $\SLE_{\kappa}(\rho,\nu)$ process can be obtained by weighting the law of ordinary $\SLE_{\kappa}$, see \cite[Theorem 6]{SchrammWilsonSLECoordinatechanges}:
\begin{lemma}
Fix $\kappa\in (0,8)$ and $0<x<y$. Let $\eta$ be an $\SLE_{\kappa}$ in $\HH$ from 0 to $\infty$ and $(g_t,t\ge 0)$ be the corresponding family of conformal maps. Define 
\begin{align*}
M_t(x,y)&=g_t'(x)^{\rho(\rho+4-\kappa)/(4\kappa)}(g_t(x)-W_t)^{\rho/\kappa}\\
&\times g_t'(y)^{\nu(\nu+4-\kappa)/(4\kappa)}(g_t(y)-W_t)^{\nu/\kappa}\times (g_t(y)-g_t(x))^{\rho\nu/(2\kappa)}.
\end{align*}
Then $M_t(x,y)$ is a local martingale for $\SLE_{\kappa}$ and the law of $\SLE_{\kappa}$ weighted by $M_t(x,y)$ is equal to the law of $\SLE_{\kappa}(\rho,\nu)$ with force points $(x,y)$ up to the swallowing time of $x$. 
\begin{comment}In particular, 
\[dM_t=M_t\left(\frac{\rho/\kappa}{W_t-V^x_t}+\frac{\nu/\kappa}{W_t-V^y_t}\right)dW_t.\]
\end{comment}
\end{lemma}


==> tex/pre_space_curves.tex <==
A planar curve is a continuous mapping from $[0,1]$ to $\C$ modulo reparameterization. Let $X$ be the set of planar curves. The metric $d$ on $X$ is defined by 
\[d(\eta_1,\eta_2)=\inf_{\varphi_1,\varphi_2}\sup_{t\in[0,1]}|\eta_1(\varphi_1(t))-\eta_2(\varphi_2(t))|,\]
where the inf is over increasing homeomorphisms $\varphi_1,\varphi_2:[0,1]\to [0,1]$. The metric space $(X, d)$ is complete and separable. A simple curve is a continuous injective mapping from $[0,1]$ to $\C$ modulo reparameterization. 
Let $X_{\simple}$ be the subspace of simple curves and denote by $X_0$ its closure. The curves in $X_0$ may have multiple points but they do not have self-crossings. 

We call $(\Omega; x,y)$ a \textit{Dobrushin domain} if $\Omega$ is a non-empty simply connected proper subset of $\C$ and $x,y$ are two distinct boundary points. Denote by $(xy)$ the arc of $\partial\Omega$ from $x$ to $y$ counterclockwise. Given a Dobrushin domain $(\Omega; x,y)$, let $X_{\simple}(\Omega; x,y)$ be the space of simple curves $\eta$ such that \[\eta(0)=x, \quad\eta(1)=y,\quad\eta(0,1)\subset\Omega.\]
Denote by $X_0(\Omega; x,y)$ the closure of $X_{\simple}(\Omega; x,y)$. 

We call $(\Omega; a, b, c, d)$ a \textit{quad (or topological rectangle)} if $\Omega$ a non-empty simply connected proper subset of $\C$ and $a, b, c, d$ are four distinct boundary points in counterclockwise order. Given a quad $(\Omega; x^L, x^R, y^R, y^L)$ and $\eps>0$, let $X_0^{\eps}(\Omega; x^L, x^R, y^R, y^L)$ be the set of pairs of curves $(\eta^L, \eta^R)$ such that 
\begin{itemize}
\item $\eta^L\in X_0(\Omega; x^L, y^L)$ and $\eta^R\in X_0(\Omega; x^R, y^R)$;
\item $\dist(\eta^L, (x^Ry^R))\ge \eps$ and $\eta^R$ is contained in the closure of the connected component of $\Omega\setminus \eta^L$ with $(x^Ry^R)$ on the boundary;
\item $\dist(\eta^R, (y^Lx^L))\ge \eps$ and $\eta^L$ is contained in the closure of the connected component of $\Omega\setminus \eta^R$ with $(y^Lx^L)$ on the boundary.
\end{itemize}
Define the metric on $X_0^{\eps}(\Omega; x^L, x^R, y^R, y^L)$ by 
\[\LD((\eta^L_1, \eta^R_1), (\eta^L_2,\eta^R_2))=\max\{d(\eta^L_1,\eta^L_2), d(\eta^R_1,\eta^R_2)\}. \]
One can check $\LD$ is a metric and the space $X_0^{\eps}(\Omega; x^L, x^R, y^R, y^L)$ with $\LD$ is complete and separable. 
Finally, set 
\[X_0(\Omega; x^L, x^R, y^R, y^L)=\bigcup_{\eps>0}X_0^{\eps}(\Omega; x^L, x^R, y^R, y^L).\]
Note that $X_0(\Omega; x^L, x^R, y^R, y^L)$ is no longer complete. 

==> tex/slepair.tex <==
\subsection{Proof of Theorem \ref{thm::slepair_lessthan4}---Uniqueness}
\begin{proposition}\label{prop::slepair_uniqueness_general}
Fix a quad $(\Omega; x^L, x^R, y^R, y^L)$ and $\kappa\in (0,8), \rho^L>-2,\rho^R>-2,\nu\ge\kappa/2-2$. 
There exists at most one probability measure on pairs of curves $(\eta^L;\eta^R)$ in $X_0(\Omega; x^L, x^R, y^R, y^L)$ with the following property: the conditional law of $\eta^R$ given $\eta^L$ is $\SLE_{\kappa}(\nu;\rho^R)$ with force points $(x^R_-;x^R_+)$ in the connected component of $\Omega\setminus\eta^L$ with $(x^Ry^R)$ on the boundary, and the conditional law of $\eta^L$ given $\eta^R$ is $\SLE_{\kappa}(\rho^L;\nu)$ with force points $(x^L_-;x^L_+)$ in the connected component of $\Omega\setminus \eta^R$ with $(y^Lx^L)$ on the boundary. 
\end{proposition}
This proposition was proved for $\kappa\in (0,4], \nu=0$ in \cite[Theorem 4.1]{MillerSheffieldIG2} and the same proof works as long as the two curves do not hit each other. To be self-contained, we will give a brief proof here and point out why this proof only works when the two curves do not hit.

Before proving this proposition, let us first explain that the conclusion for $\kappa\in (4,8)$ follows easily from the conclusion for $\kappa\in (0,4]$. Assume the conclusion in Proposition \ref{prop::slepair_uniqueness_general} is true for $\kappa\in (0,4]$. Fix $\kappa'\in (4,8)$ and set $\kappa=16/\kappa'\in (2,4)$. Suppose that $(\eta^L;\eta^R)$ is a pair in $X_0(\Omega; x^L, x^R, y^L, y^R)$ such that the conditional law of $\eta^R$ given $\eta^L$ is $\SLE_{\kappa'}(\nu;\rho^R)$ and the conditional law of $\eta^L$ given $\eta^R$ is $\SLE_{\kappa'}(\rho^L;\nu)$ where $\rho^L, \rho^R>-2$ and $\nu\ge\kappa'/2-2$. Let $\eta^L_-$ be the right boundary of $\eta^L$ and let $\eta^R_+$ be the left boundary of $\eta^R$. Since the conditional law of $\eta^R$ given $\eta^L_-$ is $\SLE_{\kappa'}(\nu;\rho^R)$, we know that the conditional law of  $\eta^R_+$ given $\eta^L_-$ is 
\[\SLE_{\kappa}(\kappa-4+\kappa\nu/4; \kappa/2-2+\kappa\rho^R/4).\]
Similarly, the conditional law of $\eta^L_-$ given $\eta^R_+$ is 
\[\SLE_{\kappa}(\kappa/2-2+\kappa\rho^L/4; \kappa-4+\kappa\nu/4).\]
Note that 
\[\kappa/2-2+\kappa\rho^L/4>-2,\quad \kappa/2-2+\kappa\rho^R/4>-2,\quad \kappa-4+\kappa\nu/4\ge \kappa/2-2.\]
By the conclusion in Proposition \ref{prop::slepair_uniqueness_general} for $\kappa\le 4$, we know that there is at most one probability measure on the pair $(\eta^L_-; \eta^R_+)$. Given the pair $(\eta^L_-; \eta^R_+)$, there is only way to reconstruct the pair $(\eta^L;\eta^R)$, since the conditional law of $\eta^L$ given $(\eta^L_-;\eta^R_+)$ is $\SLE_{\kappa'}(\rho^L; \kappa'/2-4)$; and the conditional law of $\eta^R$ given $(\eta^L_-; \eta^R_+)$ is $\SLE_{\kappa'}(\kappa'/2-4; \rho^R)$. This implies that the conclusion in Proposition \ref{prop::slepair_uniqueness_general} holds for $\kappa'\in (4,8)$. 
\begin{proof}[Proof of Proposition \ref{prop::slepair_uniqueness_general}]
From the above argument, we only need to prove the conclusion for $\kappa\in (0,4]$. 
Define a Markov chain which transitions from a configuration $(\eta^L;\eta^R)$ to another $(\tilde{\eta}^L;\tilde{\eta}^R)$ in the following way: 
Given a configuration $(\eta^L;\eta^R)$ of non-intersecting curves in $X_0(\Omega; x^L, x^R, y^R, y^L)$, we pick $q\in\{L, R\}$ uniformly and resample $\eta^q$ according to the conditional law of $\eta^q$ given the other one. We will argue that this chain has at most one stationary measure. 
Suppose that $\mu$ is any stationary measure for this chain. Fix $\eps>0$ small, and let $\mu_{\eps}$ be the measure $\mu$ conditioned on $X_0^{\eps}(\Omega; x^L, x^R, y^R, y^L)$. Then $\mu_{\eps}$ is stationary for the $\eps$-Markov chain: the chain is defined the same as before except in each step we resample the path conditioned on $X_0^{\eps}(\Omega; x^L, x^R, y^R, y^L)$. Let $\Sigma^{\eps}$ be the set of all such stationary measures. Clearly, $\Sigma^{\eps}$ is convex. 
\smallbreak
\textit{First}, we argue that $\Sigma^{\eps}$ is compact. Suppose that $\nu_n$ is a sequence in $\Sigma^{\eps}$ converging weakly to $\nu$, we need to show that $\nu$ is also stationary for the $\eps$-Markov chain. Suppose that $(\eta^L_n;\eta^R_n)$ has law $\nu_n$ and $(\eta^L;\eta^R)$ has law $\nu$. By Skorohod Representation Theorem, we could couple all $(\eta^L_n;\eta^R_n)$ and $(\eta^L;\eta^R)$ in a common space so that $\eta^L_n\to \eta^L$ and $\eta^R_n\to\eta^R$ almost surely. Let $D_n^R$ be the connected component of $\Omega\setminus\eta^L_n$ with $(x^Ry^R)$ on the boundary; and $D_n^L$ be the connected component of $\Omega\setminus\eta^R_n$ with $(y^Lx^L)$ on the boundary. Define $D^L, D^R$ for $(\eta^L;\eta^R)$ similarly. For $\delta>0$ small, let $U^R_{\delta}$ be the open set of points in $D^R$ that has distance at least $\delta$ to $\eta^L$ and define $U^L_{\delta}$ in a similar way. For $q\in\{L, R\}$, let $\LF^q=\sigma(\eta^q_n,\eta^q, n\ge 1)$. By the convergence of $\eta^q_n\to\eta^q$, we know that $U^q_n\subset D^q$ for $q\in\{L, R\}$ for $n$ large enough. 

For each $n$, let $h^L_n$ be the $\GFF$ in $D^L_n$ with the boundary value so that its flow line from $x^L$ to $y^L$ is $\SLE_{\kappa}(\rho^L;\nu)$. Define $h^R_n, h^L, h^R$ analogously. We assume that $h^L$ and $h^L_n$ for all $n$ are coupled together so that, given $\LF^R$, they are conditionally independent. The same is true for $h^R_n, h^R$.
Given $\LF^R$, the total variation distance between the law of $h^L_n$ restricted to $U^L_{\delta}$ and the law of $h^L$ restricted to $U^L_{\delta}$ tends to 0; and similar conclusion also holds for $\LF^L, h^R_n, h^R$, see \cite[Equation (4.1)]{MillerSheffieldIG2}:
\[\lim_{n\to\infty}||\LL\left[h^L_n|_{U^L_{\delta}}\cond \LF^R\right]-\LL\left[h^L|_{U^L_{\delta}}\cond \LF^R\right]||_{TV}=0,\quad \lim_{n\to\infty}||\LL\left[h^R_n|_{U^R_{\delta}}\cond \LF^L\right]-\LL\left[h^R|_{U^R_{\delta}}\cond \LF^L\right]||_{TV}=0.\]
We will deduce that, given $\LF^L$, the flow line from $x^R$ to $y^R$ generated by $h_n^R$ converges to the one generated by $h^R$. Fix $\eps'>0$, since $\nu\ge\kappa/2-2$, there exists $\delta>0$ such that, given $\LF^L$, the flow line $\eta^R$ generated by $h^R$ is contained in $U^R_{\delta}$ with probability at least $1-\eps'$ (This is the part of proof that requires the two curves to be non-intersecting).
By the total variation convergence, we could choose $n_0$ such that, for $n\ge n_0$,  
\[||\LL\left[h^R_n|_{U^R_{\delta}}\cond \LF^L\right]-\LL\left[h^R|_{U^R_{\delta}}\cond \LF^L\right]||_{TV}\le \eps'.\]
Since the flow lines are deterministic function of the $\GFF$, the total variation distance between the two flow lines given $\LF^L$ is at most $2\eps'$. This implies that, given $\LF^L$, the total variation distance between the flow line generated by $h_n^R$ converges to the one generated by $h^R$. Similar result also holds for $\LF^R, h^L_n, h^L$. Since total variation convergence implies weak convergence, we have that the transition kernel for the $\eps$-Markov chain is continuous. Therefore, the measure $\nu$ is stationary. This completes the proof that $\Sigma^{\eps}$ is compact.   
\smallbreak
\textit{Second}, we show that $\Sigma^{\eps}$ is characterized by its extremals. Since $\Sigma^{\eps}$ is compact and the space of probability measures on $X^{\eps}_0(\Omega; x^L, y^L, y^R, x^R)$ is complete and separable, Choquet's Theorem \cite[Section 3]{Choquet} implies that $\mu_{\eps}$ can be uniquely expressed as a superposition of extremals in $\Sigma^{\eps}$. To show that $\Sigma^{\eps}$ consists of at most one element, it suffices to show that there is only one such extremal in $\Sigma^{\eps}$. Suppose that $\nu,\tilde{\nu}$ are two distinct extremal elements in $\Sigma^{\eps}$. Lebesgue's Decomposition Theorem tells that there is a unique decomposition $\nu=\nu_0+\nu_1$ where $\nu_0$ is absolutely continuous with respect to $\tilde{\nu}$ and $\nu_1$ is singular to $\tilde{\nu}$. If both $\nu_0,\nu_1$ are non-zero, then they can be normalized to probability measures in $\Sigma^{\eps}$, this contradicts that $\nu$ is extremal. Therefore, either $\nu$ is absolutely continuous with respect to $\tilde{\nu}$ or $\nu$ is singular to $\tilde{\nu}$. 
We could argue that $\nu$ can not be absolutely continuous with respect to $\tilde{\nu}$. This is proved in \cite[Proof of Theorem 4.1]{MillerSheffieldIG2}. 
\smallbreak
\textit{Finally,} we only need to show that $\nu$ and $\tilde{\nu}$ can not be singular. Suppose that we have two initial configurations $(\eta_0^L;\eta_0^R)\sim \nu$ and $(\tilde{\eta}_0^L;\tilde{\eta}_0^R)\sim \tilde{\nu}$ sampled independently. First, we set $\eta^L_1=\eta^L_0$ and $\tilde{\eta}^L_1=\tilde{\eta}^L_0$, and then, given $\eta^L_1$ and $\tilde{\eta}^L_1$, we sample $\eta^R_1$ and $\tilde{\eta}^R_1$ according to the conditional law and couple them to maximize the probability for them to be equal. The fact that this probability is positive is guaranteed by Lemma \ref{lem::sle_close_positive}. Next, we set $\eta^R_2=\eta^R_1$ and $\tilde{\eta}^R_2=\tilde{\eta}^R_1$, and then, given $\eta^R_2, \tilde{\eta}^R_2$, we sample $\eta^L_2, \tilde{\eta}^L_2$ according to the conditional law and couple them to maximize the probability for them to be equal. Lemma \ref{lem::sle_close_positive} guarantees that the probability for $(\eta^L_2;\eta^R_2)=(\tilde{\eta}^L_2;\tilde{\eta}^R_2)$ is positive, which implies that $\nu$ and $\tilde{\nu}$ can not be singular. This completes the proof that $\Sigma^{\eps}$ contains at most one element. Since this is true for any $\eps>0$, we know that there is at most one stationary measure for the original Markov chain.  
\end{proof}
\begin{lemma}\label{lem::sle_close_positive}
Let $(D; x,y)$ and $(\tilde{D}; x,y)$ be two Dobrushin domains such that $\partial \tilde{D}$ agrees with $\partial D$ in neighborhoods of the arc $(xy)$. Fix $\kappa>0, \rho^L>(\kappa/2-4)\vee -2$ and $\rho^R>-2$. Let $\eta$ (resp. $\tilde{\eta}$) be an $\SLE_{\kappa}(\rho^L;\rho^R)$ in $D$ (resp. $\tilde{D}$) from $x$ to $y$ with force points $(x_-;x_+)$. Then there exists a coupling $(\eta, \tilde{\eta})$ such that the probability for them to be equal is positive. 
\end{lemma}
\begin{proof}
Proof of \cite[Lemma 4.2]{MillerSheffieldIG2} and the discussion after the proof there. 
\end{proof}

\subsection{Proof of Theorem \ref{thm::slepair_lessthan4}---Identification}
The identification of Theorem \ref{thm::slepair_lessthan4} was implicitly proved in \cite{LawlerPartitionFunctionsSLE, KozdronLawlerMultipleSLEs}. We will give a complete proof here and give necessary references. 

Suppose $K$ is an $\HH$-hull such that $\dist(0,K)>0$ and let $H:=\HH\setminus K$. Let $\phi$ be the conformal map from $H$ onto $\HH$ such that $\phi(0)=0$ and $\lim_{z\to\infty}\phi(z)/z=1$.
We wish to compare the law of $\SLE_{\kappa}$ in $\HH$ and the law of $\SLE_{\kappa}$ in $H$. 
Suppose $\eta$ is an $\SLE_{\kappa}$ in $\HH$ from 0 to $\infty$ and $(g_t,t\ge 0)$ is the corresponding family of conformal maps. Let $T$ be the first time that $\eta$ hits $K$.  We will study the law of $\tilde{\eta}(t)=\phi(\eta(t))$ for $t<T$. Define $\tilde{g}_t$ to be the conformal map from $\HH\setminus\tilde{\eta}[0,t]$ onto $\HH$ normalized at $\infty$ and let $h_t$ be the conformal map from $\HH\setminus g_t(K)$ onto $\HH$ such that $h_t\circ g_t=\tilde{g}_t\circ\phi$, see \cite[Section 5]{LawlerSchrammWernerConformalRestriction}. Note that $\tilde{W}_t=h_t(W_t)$ is the driving function for $\tilde{\eta}$ and 
\begin{equation}\label{eqn::sle_domain_driving}
d\tilde{W}_t=h_t'(W_t)dW_t+(\kappa/2-3)h_t''(W_t)dt.
\end{equation}
\textit{Schwarzian derivative} for a conformal map $f$ is defined to be 
\[Sf(z)=\frac{f'''(z)}{f'(z)}-\frac{3f''(z)^2}{2f'(z)^2}.\]
\begin{lemma}\label{lem::sle_domain_mart}
Fix $\kappa\in (0,4]$. The following process is a uniformly integrable martingale:
\[M_t:=\one_{\{t<T\}}h'_t(W_t)^b\exp\left(-c\int_0^t\frac{Sh_s(W_s)}{6}ds\right),\quad \text{where }b=\frac{6-\kappa}{2\kappa},\quad c=\frac{(3\kappa-8)(6-\kappa)}{2\kappa}.\]
Moreover, the law of $\eta$ weighted by $M$ is the same as the law of $\SLE_{\kappa}$ in $H$ from 0 to $\infty$. 
\end{lemma}
\begin{proof}
One can check by It\^{o}'s Formula that $M$ is a local martingale (see the calculation in \cite[Section 5]{LawlerSchrammWernerConformalRestriction}) and we have 
\[dM_t=bM_t\frac{h_t''(W_t)}{h_t'(W_t)}dW_t.\]
Let $\tilde{\PP}$ denote the law of $\eta$ weighted by $M$. Suppose that $B$ is the Brownian motion in $\PP$ and $W_t=\sqrt{\kappa}B_t$, then 
\[\tilde{B}_t=B_t+\int_0^t(\kappa/2-3)\frac{h_s''(W_s)}{h_s'(W_s)}ds\]
is the Brownian motion under $\tilde{\PP}$. Compare this with (\ref{eqn::sle_domain_driving}), we see that $d\tilde{W}_t=\sqrt{\kappa}h_t'(W_t)d\tilde{B}_t$. Let $s=s(t)$ be the capacity of $\tilde{\eta}[0,t]$, then we have $\dot{s}(t)=h_t'(W_t)^2$. Thus, after the time change, we have $d\tilde{W}_s=\sqrt{\kappa}d\tilde{B}_s$. This implies that the law of $\eta$ weighted by $M$ is the same as the law of $\SLE_{\kappa}$ in $H$ up to the first time that $\eta$ hits $K$. At the same time, we know that $\SLE_{\kappa}$ in $H$ will never hits the boundary (except at the end points) when $\kappa\in (0,4]$. Hence, $M$ is actually a uniformly integrable martingale and the law of $\eta$ weighted by $M$ is the same as the law of $\SLE_{\kappa}$ in $H$ for all time. 
\end{proof}
Consider the martingale in Lemma \ref{lem::sle_domain_mart}, since $h_t'(W_t)\to 1$ as $t\to\infty$ on $\{T=\infty\}$, we have 
\[M_{\infty}:=\lim_{t\to\infty} M_t=\one_{\{T=\infty\}}\exp\left(-c\int_0^{\infty}\frac{Sh_s(W_s)}{6}ds\right).\]
We will discuss the quantity in the right hand side. The \textit{Brownian loop measure} is the measure on unrooted Brownian loops. Since we do not need to do calculation with it, we omit the introduction to Brownian loop measure here and refer \cite[Sections 3,4]{LawlerWernerBrownianLoopsoup} for a clear definition. Given a non-empty simply connected domain $\Omega\subsetneq\C$ and two disjoint subsets $V_1, V_2$, denote by $m(\Omega; V_1, V_2)$ the Brownian loop measure of loops in $\Omega$ that intersect both $V_1$ and $V_2$. This quantity is conformal invariant: $m(f(\Omega); f(V_1), f(V_2))=m(\Omega; V_1, V_2)$ for any conformal transformation $f$ on $\Omega$. When both of $V_1, V_2$ are closed, one of them is compact and $\dist(V_1, V_2)>0$, we have $0<m(\Omega; V_1, V_2)<\infty$. It is proved in \cite[Equation (22)]{LawlerWernerBrownianLoopsoup} that$-(1/6)\int_0^{t}Sh_s(W_s)6ds=m(\HH; K, \eta[0,t])$.
Thus we have
\begin{equation}\label{eqn::sle_domain_brownianloopmass}
M_{\infty}=\one_{\{T=\infty\}}\exp\left(-c\int_0^{\infty}\frac{Sh_s(W_s)}{6}ds\right)=\one_{\{T=\infty\}}\exp(c m(\HH; K, \eta)).
\end{equation}
\begin{proof}[Proof of Theorem \ref{thm::slepair_lessthan4}, Identification] There are three steps: first, we construct a probability measure $\PP$ on pairs of curves; second, we show that this probability measure has the property in ``Uniqueness"; last, we show that the marginal law of $\eta^L$ under $\PP$ is $\hSLE_{\kappa}$. 
\smallbreak
\textit{First}, we will construct a probability measure on $(\eta^L;\eta^R)$. 
Fix $\kappa\in (0,4]$ and $0<x<y$. By conformal invariance, it is sufficient to give the construction for the quad $(\HH; 0,x,y,\infty)$. 
Denote by $\PP_L$ the law of $\SLE_{\kappa}$ in $\HH$ from 0 to $\infty$ and denote by $\PP_R$ the law of $\SLE_{\kappa}$ in $\HH$ from $x$ to $y$. Define the measure $\mu$ on $X_0(\HH; 0,x,y,\infty)$ by 
\[\mu[d\eta^L, d\eta^R]=\one_{\{\eta^L\cap\eta^R=\emptyset\}}\exp\left(c m(\HH; \eta^L, \eta^R)\right)\PP_L\left[d\eta^L\right]\otimes\PP_R\left[d\eta^R\right].\] 
We argue that the total mass of $\mu$, denoted by $|\mu|$, is finite. Given $\eta^L\in X_0(\HH; 0,\infty)$, let $g$ be any conformal map from the connected component of $\HH\setminus \eta^L$ with $(xy)$ on the boundary onto $\HH$, then we have
\begin{align*}
|\mu|&=\E_L\otimes\E_R\left[\one_{\{\eta^L\cap\eta^R=\emptyset\}}\exp\left(c m(\HH; \eta^L, \eta^R)\right)\right]\\
&=\E_L\left[\left(\frac{g'(x)g'(y)}{(g(x)-g(y))^2}\right)^b\right]\tag{By Lemma \ref{lem::sle_domain_mart} and (\ref{eqn::sle_domain_brownianloopmass})}\\
&=(x-y)^{-2b}(x/y)^{2/\kappa}F(x/y).\tag{By Proposition \ref{prop::hypersle_mart}}
\end{align*}
This implies that $|\mu|$ is positive finite. We define the probability measure $\PP$ to be $\mu/|\mu|$. 
\smallbreak
\textit{Second}, we show that, under $\PP$, the conditional law of $\eta^R$ given $\eta^L$ is $\SLE_{\kappa}$. By the symmetry in the definition of $\PP$, we know that the conditional law of $\eta^L$ given $\eta^R$ is also $\SLE_{\kappa}$ and hence $\PP$ satisfies the property in ``Uniqueness". Given $\eta^L$, denote by $H$ the connected component of $\HH\setminus \eta^L$ with $(xy)$ on the boundary and let $g$ be any conformal map from $H$ onto $\HH$. Denote by $\PP_R$ the law of $\SLE_{\kappa}$ in $\HH$ from $x$ to $y$ and by $\tilde{\PP}_R$ the law of $\SLE_{\kappa}$ in $H$ from $x$ to $y$. By Lemma \ref{lem::sle_domain_mart},
for any bounded continuous functional $F$ on continuous curves, we have 
\begin{align*}
\E\left[F(\eta^R)\cond \eta^L\right]&=|\mu|^{-1}\E_R\left[\one_{\{\eta^L\cap\eta^R=\emptyset\}}\exp\left(c m(\HH; \eta^L, \eta^R)\right)F(\eta^R)\right]\\
&=|\mu|^{-1}\left(\frac{g'(x)g'(y)}{(g(x)-g(y))^2}\right)^b\tilde{\E}_R\left[F(\eta^R)\right].
\end{align*}
This implies that the conditional law of $\eta^R$ given $\eta^L$ is $\SLE_{\kappa}$ in $H$. 
\smallbreak
\textit{Finally}, we show that, under $\PP$, the marginal law of $\eta^L$ is $\hSLE_{\kappa}$. In fact, the above equation implies that the law of $\eta^L$ is the law of $\SLE_{\kappa}$ in $\HH$ from 0 to $\infty$ weighted by \[\left(\frac{g'(x)g'(y)}{(g(x)-g(y))^2}\right)^b.\]
Therefore, by Proposition \ref{prop::hypersle_mart} and the argument in its proof, we see that the law of $\eta^L$ coincides with $\hSLE_{\kappa}$ as desired.
\end{proof}

\begin{figure}[ht!]
\begin{center}
\includegraphics[width=0.45\textwidth]{figures/slepair_levellines}
\end{center}
\caption{\label{fig::slepair_levellines} Let $\eta^L$ be the level line of $h+\lambda$ and $\eta^R$ be the level line of $h-\lambda$. Then the pair $(\eta^L;\eta^R)$ is the unique pair in Theorem \ref{thm::slepair_lessthan4} for $\kappa=4$.}
\end{figure}

\begin{remark}\label{rem::slepair_lessthan4_degenerate}
[Degenerate case in Theorem \ref{thm::slepair_lessthan4}---level lines of $\GFF$]
When $\kappa=4$, the SDE (\ref{eqn::hyperSLE_sde}) degenerates to the SDE (\ref{eqn::sle_rho_sde}).  In other words, $\hSLE_4$ in $\HH$ with marked points $(x,y)$ is the same as $\SLE_4(2,-2)$ with force points $(x,y)$. In this degenerate case, the pair of curves in Theorem \ref{thm::slepair_lessthan4} can be realized by a pair of level lines of $\GFF$. 
Fix a quad $(\Omega; x^L, y^L, y^R, x^R)$. Let $h$ be the $\GFF$ on $\Omega$ with the following boundary data (see Figure \ref{fig::slepair_levellines}):
$-2\lambda$ on $(y^Lx^L)$, $0$ on $(x^Lx^R)\cup(y^Ry^L)$, and $2\lambda$ on $(x^Ry^R)$.
Let $\eta^L$ be the level line of $h$ with height $-\lambda$ and let $\eta^R$ be the level line of $h$ with height $\lambda$. Then we have that the marginal law of $\eta^L$ is $\SLE_4(2,-2)$ with force points $(x^R, y^R)$ and the conditional law of $\eta^L$ given $\eta^R$ is $\SLE_4$; the marginal law of $\eta^R$ is $\SLE_4(2,-2)$ with force points $(x^L, y^L)$ and the conditional law of $\eta^R$ given $\eta^L$ is $\SLE_4$. Thus the pair $(\eta^L;\eta^R)$ is the unique pair described in Theorem \ref{thm::slepair_lessthan4} for $\kappa=4$. 
\end{remark}

\subsection{Proof of Theorem \ref{thm::slepair_greaterthan4}}
We will show the existence in Theorem \ref{thm::slepair_greaterthan4} by checking directly that the law given in the identification part satisfies the property in the uniqueness part. We only need to show it for $\HH$. Recall that $\kappa, \kappa', \lambda,\chi$ are defined in (\ref{eqn::gff_constants}). 
\textit{First}, the conclusion for $\kappa<4$ can be checked by flow lines of $\GFF$. Fix the domain $(\HH; x^L, x^R, \infty)$ with $x^L<x^R$. 
Suppose $h$ is a $\GFF$ with the following boundary data: $-2\lambda$ on $(-\infty, x^L)$, $0$ on $(x^L, x^R)$, and $2\lambda$ on $(x^R, \infty)$. Set $\theta=\lambda/\chi$. Let $\eta^L$ be the flow line of $h$ with angle $\theta$ and let $\eta^R$ be the flow line of $h$ with angle $-\theta$. Then we have that the law of $\eta^L$ is $\SLE_{\kappa}(2)$ with force point $x^R$; and that the law of $\eta^L$ given $\eta^R$ is $\SLE_{\kappa}$ as desired. 
\textit{Second}, when $\kappa=4$, see Remark \ref{rem::slepair_lessthan4_degenerate} and take $y^L=y^R=\infty$. \textit{Thirdly}, fix $\kappa'\in (4,8)$ and $\kappa=16/\kappa\in (2,4)$ and we check the conclusion by counterflow lines of $\GFF$. Fix the domain $(\HH; x^L, x^R, 0)$ where $x^R<0<x^L$ (no typo here). 
Suppose $h$ is a $\GFF$ with the following boundary data (see Figure \ref{fig::slepair_counterflowlines}): 
\[\pi\chi\text{ on }(-\infty, x^R),\quad -2\lambda+2\pi\chi\text{ on }(x^R, 0),\quad 2\lambda-2\pi\chi\text{ on }(0,x^L),\quad -\pi\chi\text{ on }(x^L,\infty).\]
Set $\theta_1=\lambda(\kappa/2-1)/\chi$ and $\theta_2=\lambda/\chi$. Note that $\theta_2-\theta_1=\pi$. Let $\eta^L_-$ be the flow line of $h$ with angle $-\theta_2$, let $\eta^L_+$ be the flow line of $h$ with angle $-\theta_1$, let $\eta^R_-$ be the flow line of $h$ with angle $\theta_1$, and let $\eta^R_+$ be the flow line of $h$ with angle $\theta_2$. Finally, given the pair $\eta^L_+$ and $\eta^L_-$, let $\eta^L$ be the $\SLE_{\kappa'}(\kappa'/2-4;\kappa'/2-4)$ from $x^L$ to $0$ lying between $\eta^L_+$ and $\eta^L_-$; and given the pair $\eta^R_+$ and $\eta^R_-$, let $\eta^R$ be the $\SLE_{\kappa'}(\kappa'/2-4;\kappa'/2-4)$ from $x^R$ to $0$ lying between $\eta^R_+$ and $\eta^R_-$. Consider the pair $(\eta^L;\eta^R)$:
\begin{itemize}
\item Given $\eta^R_-$, the conditional law of $\eta^L_+$ is $\SLE_{\kappa}(\kappa-4;\kappa/2-2)$, and the conditional law of $\eta^L_-$ is $\SLE_{\kappa}(\kappa/2-2;\kappa-4)$. 
\item Given the pair $\eta^L_+$ and $\eta^L_-$, the conditional law of $\eta^L$ is $\SLE_{\kappa'}(\kappa'/2-4;\kappa'/2-4)$.
\end{itemize}
Combining these two facts with Lemma \ref{lem::counterflowline_decomposition}, we know that the conditional law of $\eta^L$ given $\eta^R_-$ is $\SLE_{\kappa'}$. Therefore, the conditional law of $\eta^L$ given $\eta^R$ is $\SLE_{\kappa'}$. Similarly, the conditional law of $\eta^R$ given $\eta^L$ is $\SLE_{\kappa'}$. Thus the pair $(\eta^L;\eta^R)$ satisfies the property in the uniqueness part of Theorem \ref{thm::slepair_greaterthan4}.

\begin{figure}[ht!]
\begin{center}
\includegraphics[width=0.45\textwidth]{figures/slepair_counterflowlines}
\end{center}
\caption{\label{fig::slepair_counterflowlines} Let $\eta^L$ be the $\SLE_{\kappa'}(\kappa'/2-4;\kappa'/2-4)$ from $x^L$ to $0$ lying between $\eta^L_+$ and $\eta^L_-$ (in the grey part); and let $\eta^R$ be the $\SLE_{\kappa'}(\kappa'/2-4;\kappa'/2-4)$ from $x^R$ to $0$ lying between $\eta^R_+$ and $\eta^R_-$ (in the grey part). Then the pair $(\eta^L;\eta^R)$ satisfies the following property: the conditional law of $\eta^L$ given $\eta^R$ is $\SLE_{\kappa'}$ and the conditional law of $\eta^R$ given $\eta^R$ is $\SLE_{\kappa'}$. }
\end{figure}


\smallbreak
{\color{red}To complete the proof of Theorem \ref{thm::slepair_greaterthan4}, we only need to show the uniqueness. }



==> tex/slepair_greaterthan4.tex <==

We will show the existence in Theorem \ref{thm::slepair_greaterthan4} by checking directly that the law given in the identification part satisfies the property in the uniqueness part. We only need to show it for $\HH$. Recall that $\kappa, \kappa', \lambda,\chi$ are defined in (\ref{eqn::gff_constants}). 
\textit{First}, the conclusion for $\kappa<4$ can be checked by flow lines of $\GFF$. Fix the domain $(\HH; x^L, x^R, \infty)$ with $x^L<x^R$. 
Suppose $h$ is a $\GFF$ with the following boundary data: $-2\lambda$ on $(-\infty, x^L)$, $0$ on $(x^L, x^R)$, and $2\lambda$ on $(x^R, \infty)$. Set $\theta=\lambda/\chi$. Let $\eta^L$ be the flow line of $h$ with angle $\theta$ and let $\eta^R$ be the flow line of $h$ with angle $-\theta$. Then we have that the law of $\eta^L$ is $\SLE_{\kappa}(2)$ with force point $x^R$; and that the law of $\eta^L$ given $\eta^R$ is $\SLE_{\kappa}$ as desired. 
\textit{Second}, when $\kappa=4$, see Remark \ref{rem::slepair_lessthan4_degenerate} and take $y^L=y^R=\infty$. \textit{Thirdly}, fix $\kappa'\in (4,8)$ and $\kappa=16/\kappa\in (2,4)$ and we check the conclusion by counterflow lines of $\GFF$. Fix the domain $(\HH; x^L, x^R, 0)$ where $x^R<0<x^L$ (no typo here). 
Suppose $h$ is a $\GFF$ with the following boundary data (see Figure \ref{fig::slepair_counterflowlines}): 
\[\pi\chi\text{ on }(-\infty, x^R),\quad -2\lambda+2\pi\chi\text{ on }(x^R, 0),\quad 2\lambda-2\pi\chi\text{ on }(0,x^L),\quad -\pi\chi\text{ on }(x^L,\infty).\]
Set $\theta_1=\lambda(\kappa/2-1)/\chi$ and $\theta_2=\lambda/\chi$. Note that $\theta_2-\theta_1=\pi$. Let $\eta^L_-$ be the flow line of $h$ with angle $-\theta_2$, let $\eta^L_+$ be the flow line of $h$ with angle $-\theta_1$, let $\eta^R_-$ be the flow line of $h$ with angle $\theta_1$, and let $\eta^R_+$ be the flow line of $h$ with angle $\theta_2$. Finally, given the pair $\eta^L_+$ and $\eta^L_-$, let $\eta^L$ be the $\SLE_{\kappa'}(\kappa'/2-4;\kappa'/2-4)$ from $x^L$ to $0$ lying between $\eta^L_+$ and $\eta^L_-$; and given the pair $\eta^R_+$ and $\eta^R_-$, let $\eta^R$ be the $\SLE_{\kappa'}(\kappa'/2-4;\kappa'/2-4)$ from $x^R$ to $0$ lying between $\eta^R_+$ and $\eta^R_-$. Consider the pair $(\eta^L;\eta^R)$:
\begin{itemize}
\item Given $\eta^R_-$, the conditional law of $\eta^L_+$ is $\SLE_{\kappa}(\kappa-4;\kappa/2-2)$, and the conditional law of $\eta^L_-$ is $\SLE_{\kappa}(\kappa/2-2;\kappa-4)$. 
\item Given the pair $\eta^L_+$ and $\eta^L_-$, the conditional law of $\eta^L$ is $\SLE_{\kappa'}(\kappa'/2-4;\kappa'/2-4)$.
\end{itemize}
Combining these two facts with Lemma \ref{lem::counterflowline_decomposition}, we know that the conditional law of $\eta^L$ given $\eta^R_-$ is $\SLE_{\kappa'}$. Therefore, the conditional law of $\eta^L$ given $\eta^R$ is $\SLE_{\kappa'}$. Similarly, the conditional law of $\eta^R$ given $\eta^L$ is $\SLE_{\kappa'}$. Thus the pair $(\eta^L;\eta^R)$ satisfies the property in the uniqueness part of Theorem \ref{thm::slepair_greaterthan4}.

\begin{figure}[ht!]
\begin{center}
\includegraphics[width=0.45\textwidth]{figures/slepair_counterflowlines}
\end{center}
\caption{\label{fig::slepair_counterflowlines} Let $\eta^L$ be the $\SLE_{\kappa'}(\kappa'/2-4;\kappa'/2-4)$ from $x^L$ to $0$ lying between $\eta^L_+$ and $\eta^L_-$ (in the grey part); and let $\eta^R$ be the $\SLE_{\kappa'}(\kappa'/2-4;\kappa'/2-4)$ from $x^R$ to $0$ lying between $\eta^R_+$ and $\eta^R_-$ (in the grey part). Then the pair $(\eta^L;\eta^R)$ satisfies the following property: the conditional law of $\eta^L$ given $\eta^R$ is $\SLE_{\kappa'}$ and the conditional law of $\eta^R$ given $\eta^R$ is $\SLE_{\kappa'}$. }
\end{figure}


\smallbreak
{\color{red}To complete the proof of Theorem \ref{thm::slepair_greaterthan4}, we only need to show the uniqueness. }


